Automated decision-making for dynamic task assignment at scale

The Dynamic Task Assignment Problem (DTAP) concerns matching resources to tasks in real time while minimizing some objectives, like resource costs or task cycle time. In this work, we consider a DTAP variant where every task is a case composed of a stochastic sequence of activities. The DTAP, in this case, involves the decision of which employee to assign to which activity to process requests as quickly as possible. In recent years, Deep Reinforcement Learning (DRL) has emerged as a promising tool for tackling this DTAP variant, but most research is limited to solving small-scale, synthetic problems, neglecting the challenges posed by real-world use cases. To bridge this gap, this work proposes a DRL-based Decision Support System (DSS) for real-world scale DTAPS. To this end, we introduce a DRL agent with two novel elements: a graph structure for observations and actions that can effectively represent any DTAP and a reward function that is provably equivalent to the objective of minimizing the average cycle time of tasks. The combination of these two novelties allows the agent to learn effective and generalizable assignment policies for real-world scale DTAPs. The proposed DSS is evaluated on five DTAP instances whose parameters are extracted from real-world logs through process mining. The experimental evaluation shows how the proposed DRL agent matches or outperforms the best baseline in all DTAP instances and generalizes on different time horizons and across instances.

==> OLD_06_results.tex <==
\subsection{Results}\label{subsec:results}

The simulations detailed in \cref{sec:experimental_setting} are utilized to train the DRL agent on 7-day traces. The trained agent is then applied to a set of 1000 independent 7-day traces. For each trace, the average cycle time is recorded. The means and 95\% confidence intervals of the average cycle times are reported in~\cref{tab:results_7d}. We compare the results of the DRL approach (PPO) against three baseline agents following simple heuristic policies: the random policy (Random), which selects assignments randomly; the First-In-First-Out (FIFO) policy, which prioritizes cases based on their entry time; and the Shortest Processing Time (SPT) policy, which assigns activities to the resource that completes them the fastest on average.

\begin{table}[ht]
\centering
\begin{tabular}{>{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm}}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{4}{c}{\textbf{Method}} \\
\cmidrule(lr){2-5}
 & \textbf{Random} & \textbf{FIFO} & \textbf{SPT} & \textbf{PPO} \\
\midrule
BPI2012 & 46.6 \(\pm\) 0.7 & 49.1 \(\pm\) 0.9 & 15.4 \(\pm\) 0.6 & 15.3 \(\pm\) 0.6 \\
BPI2017 & 10.5 \(\pm\) 0.2 & 10.3 \(\pm\) 0.2 & 7.2 \(\pm\) 0.2 & 6.2 \(\pm\) 0.1 \\
BPI2018 & 60.1 \(\pm\) 0.9 & 61.7 \(\pm\) 0.9 & 33.2 \(\pm\) 0.9 & 33.1 \(\pm\) 0.9 \\
CONS & 49.7 \(\pm\) 0.6 & 51.1 \(\pm\) 0.7 & 45.8 \(\pm\) 0.7 & 44.1 \(\pm\) 0.6 \\
PROD & 66.8 \(\pm\) 0.7 & 66.9 \(\pm\) 0.7 & 63.3 \(\pm\) 0.7 & 63.1 \(\pm\) 0.7 \\
\bottomrule
\end{tabular}
\caption{Performance comparison on $7$ day traces.}
\label{tab:results_7d}
\end{table}

The results on the $7$ day horizon instances seem to point to a substantial parity between the DRL approach and SPT, except for the BPI2017 dataset, where the DRL approach clearly outperforms SPT. To confront the two methods, we collect all the observations on $1000$ replications of $7$ days episodes for each problem. In~\cref{fig:ppo_vs_spt}, we report the percentage of observations in which PPO and SPT take the same actions (in blue) and in which they take different actions (in orange).

\begin{figure}[ht]
    \centering
    \centerline{\includegraphics[width=0.6\textwidth]{images/differences.pdf}}
    \caption{Percentage of equal (blue) and different (orange) actions between PPO and SPT on a set of 1000 observations.}
    \label{fig:ppo_vs_spt}
\end{figure}

It can be observed that the DRL agent behaves differently depending on the problem. On the two extremes, in BPI2012, PPO mimics SPT on all occasions, whereas in BPI2017 it behaves differently in more than $20\%$ of cases. This observation aligns with the results in~\cref{tab:results_7d}, where PPO notably outperforms SPT in BPI2017, but performs similarly to SPT on the other datasets. To explain this result, we report the average number of cases in the system over a $4$ week time horizon in~\cref{fig:regime} under the SPT policy.

\begin{figure}[ht]
    \centering
    \centerline{\includegraphics[width=0.7\textwidth]{images/all_problems_cases.pdf}}
    \caption{The number of cases in the system when following the SPT policy over 4 weeks.}
    \label{fig:regime}
\end{figure}

The graph in~\cref{fig:regime} highlights that, except for BPI2017, all considered systems are unstable even under an effective policy such as SPT. This observation seems to point to the fact that system stability is a prerequisite to learning policies that are better than SPT. In fact, the Shortest Remaining Processing Time (SRPT) heuristic~\cite{doi:10.1287/opre.14.4.670}, which is closely related to SPT, has been shown to minimize the mean sojourn time in single-server queue systems. An unstable multi-server system approximates a single-server system, which helps explain the effectiveness of SPT in unstable systems.

\begin{comment}
\subsection{Generalization study: extended time horizon}
\end{comment}

The instabilities observed in~\cref{fig:regime} can be explained by the fact that the DTAPs are parameterized from real-world logs using the available data, which are collected over a limited period of time. It is likely that the period considered shows higher arrival rates or lower resource availability than those experienced over longer periods in the systems that produced those logs. However, system instability does not represent a problem for optimization over a limited time horizon. The expected effect of instability is only that the average cycle times for longer time horizons should be higher than those reported in~\cref{tab:results_7d}.

To prove this claim, in~\cref{table:results_14d}, we test on a $14$ days horizon the models that were trained on a $7$ days horizon.

\begin{table}[ht]
\centering
\begin{tabular}{>{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm} >{\centering\arraybackslash}m{2cm}}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{4}{c}{\textbf{Method}} \\
\cmidrule(lr){2-5}
 & \textbf{Random} & \textbf{FIFO} & \textbf{SPT} & \textbf{PPO} \\
\midrule
BPI2012 & \(98.8 \pm 1.1\) & \(105.4 \pm 1.4\) & \(24.2 \pm 0.9\) & \(24.0 \pm 0.9\) \\
BPI2017 & \(13.6 \pm 0.3\) & \(12.9 \pm 0.2\) & \(8.4 \pm 0.1\) & \(6.9 \pm 0.1\) \\
BPI2018 & \(118.9 \pm 1.9\) & \(115.8 \pm 1.9\)  & \(69.1 \pm 1.7\) & \( 68.6 \pm 1.8\) \\
CONS & \(100.9 \pm 1.1\) & \(102.5 \pm 1.1\) & \(87.2 \pm 1.1\) & \(86.3 \pm 1.1\) \\
PROD & \(120.5 \pm 1.1\) & \(121.1 \pm 1.1\) & \(115.6 \pm 1.2\) & \(115.5 \pm 1.1\) \\
\bottomrule
\end{tabular}
\caption{Performance comparison on $14$ day traces.}
\label{table:results_14d}
\end{table}

As expected, the average cycle times registered on a $14$ day horizon are higher than those recorded on a $7$ day horizon for all unstable systems. However, the relative gap between the best policies (SPT and PPO) and the worst ones (Random, FIFO) remains substantially the same, pointing to the robustness of the learned policies when applied to longer horizons than the training ones in both stable and unstable systems.

\begin{comment}
\subsection{Generalization study: cross-dataset test}
\end{comment}

A remarkable property of GNNs is their ability to generalize across different domains. 
Given the observations reported in~\cref{fig:ppo_vs_spt}, it is interesting to report the results obtained testing PPO with the weights learned on BPI2017 on the other four datasets. 
In~\cref{table:results_generalized}, we show how the algorithm trained on each dataset performs on the DTAP instance used to train it (value on the diagonal) and on the other instances.

\begin{table}[ht]
\centering
\begin{tabular}{>{\centering\arraybackslash}m{1.8cm} >{\centering\arraybackslash}m{1.8cm} >{\centering\arraybackslash}m{1.8cm} >{\centering\arraybackslash}m{1.8cm} >{\centering\arraybackslash}m{1.8cm} >{\centering\arraybackslash}m{1.8cm}}
\toprule
\multirow{2}{*}{\makecell{\textbf{Test}\\\textbf{Dataset}}} & \multicolumn{5}{c}{\textbf{Train Dataset}} \\
\cmidrule(lr){2-6}
 & \textbf{BPI2012} & \textbf{BPI2017} & \textbf{BPI2018} & \textbf{CONS} & \textbf{PROD} \\
\midrule
BPI2012 & \(15.3 \pm 0.6\) & \(14.9 \pm 0.6\) & \(15.5 \pm 0.6\) & \(15.2 \pm 0.6\) &  \(17.2 \pm 0.7\)\\
BPI2017 & \(7.1 \pm 0.1\) & \(6.2 \pm 0.1\) & \(7.2 \pm 0.1\) & \(7.2 \pm 0.1\)  & \(7.1 \pm 0.1\)  \\
BPI2018 & \(33.2 \pm 0.8\) & \(33.4 \pm 0.8\) & \(33.1 \pm 0.9\) & \(33.4 \pm 0.8\) & \(33.9 \pm 0.9\) \\
CONS & \(44.3 \pm 0.6\) & \(44.1 \pm 0.6\) & \(44.5 \pm 0.6\) & \(44.1 \pm 0.6\) & \(44.8 \pm 0.6\) \\
PROD & \(62.9 \pm 0.7\) & \(62.8 \pm 0.7\) & \(63.8 \pm 0.7\) & \(63.3 \pm 0.7\) & \(63.1 \pm 0.7\) \\
\bottomrule
\end{tabular}
\caption{Performance of the DRL model trained on each problem applied to the others on $7$ day traces.}
\label{table:results_generalized}
\end{table}

The results in~\cref{table:results_generalized} point to the substantial robustness of the learned policies. Interestingly, the agent trained on the BPI2017 environment presented good cross-dataset results, but none of the other agents could match the original's performance when tested on BPI2017. This observation suggests that a stable training environment can lead to good generalization capabilities even in unstable environments, while the opposite is not true.
